AI as "Co-founder": GenAI for Entrepreneurship

This paper studies whether, how, and for whom generative artificial intelligence (GenAI) facilitates firm creation. Our identification strategy exploits the November 2022 release of ChatGPT as a global shock that lowered start-up costs and leverages variations across geo-coded grids with differential pre-existing AI-specific human capital. Using high-resolution and universal data on Chinese firm registrations by the end of 2024, we find that grids with stronger AI-specific human capital experienced a sharp surge in new firm formation$\unicode{x2013}$driven entirely by small firms, contributing to 6.0% of overall national firm entry. Large-firm entry declines, consistent with a shift toward leaner ventures. New firms are smaller in capital, shareholder number, and founding team size, especially among small firms. The effects are strongest among firms with potential AI applications, weaker financing needs, and among first-time entrepreneurs. Overall, our results highlight that GenAI serves as a pro-competitive force by disproportionately boosting small-firm entry.

==> main_tables/main_t1_after.tex <==
  & \multicolumn{2}{c}{Control   Group}              & \multicolumn{2}{c}{Treatment   Group}            & \multicolumn{1}{c}{Difference} \\
\multicolumn{1}{c}{} & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{Mean}       \\
% \multicolumn{2}{l}{\textbf{After ChatGPT}}          &                          &                       &                          &                                \\
\midrule
Num new firms                & 1,247,784 & 2.595  & 81,464 & 44.529 & -41.934*** \\
Num small firms              & 1,247,784 & 1.367  & 81,464 & 22.349 & -20.982*** \\
Num large firms              & 1,247,784 & 1.071  & 81,464 & 19.742 & -18.671*** \\
Num high upstream            & 1,247,784 & 0.373  & 81,464 & 11.15  & -10.778*** \\
Num low upstream             & 1,247,784 & 2.222  & 81,464 & 33.37  & -31.149*** \\
Num high downstream          & 1,247,784 & 1.073  & 81,464 & 27.72  & -26.646*** \\
Num low downstream           & 1,247,784 & 1.521  & 81,464 & 16.801 & -15.280*** \\
Num high entrep              & 1,247,784 & 1.795  & 81,464 & 38.113 & -36.318*** \\
Num low entrep               & 1,247,784 & 0.799  & 81,464 & 6.408  & -5.609***  \\
Pct serial entrep            & 457,610   & 23.722 & 50,862 & 34.458 & -10.736*** \\
Pct serial entrep small      & 457,610   & 15.293 & 50,862 & 29.155 & -13.862*** \\
Pct serial entrep large      & 457,610   & 15.707 & 50,862 & 31.001 & -15.295*** \\
Tot shareholders             & 440,811   & 1.467  & 50,186 & 1.682  & -0.215***  \\
Tot shareholders small       & 313,730   & 1.363  & 45,496 & 1.576  & -0.213***  \\
Tot shareholders large       & 291,160   & 1.61   & 45,785 & 1.804  & -0.195***  \\
Pct indiv shareholders       & 440,811   & 93.335 & 50,186 & 88.369 & 4.966***   \\
Pct indiv shareholders small & 313,730   & 96.152 & 45,496 & 92.976 & 3.176***   \\
Pct indiv shareholders large & 291,160   & 90.103 & 45,785 & 83.771 & 6.332***   \\
Exec team size               & 404,438   & 2.007  & 49,722 & 1.98   & 0.027***   \\
Exec team size small         & 274,462   & 1.938  & 44,722 & 1.931  & 0.007**    \\
Exec team size large         & 276,458   & 2.096  & 45,387 & 2.04   & 0.056***     \\
\bottomrule

==> main_tables/main_t1_before.tex <==
     & \multicolumn{2}{c}{Control Group}                & \multicolumn{2}{c}{Treatment Group}              & \multicolumn{1}{c}{Difference} \\
\multicolumn{1}{c}{}         & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{Mean}       \\
\midrule
Num new firms                & 1,247,784             & 2.259                    & 81,464                & 38.491                   & -36.232***                     \\
Num small firms              & 1,247,784             & 0.798                    & 81,464                & 12.449                   & -11.650***                     \\
Num large firms              & 1,247,784             & 1.323                    & 81,464                & 24.143                   & -22.820***                     \\
Num high upstream            & 1,247,784             & 0.315                    & 81,464                & 9.96                     & -9.645***                      \\
Num low upstream             & 1,247,784             & 1.94                     & 81,464                & 28.511                   & -26.571***                     \\
Num high downstream          & 1,247,784             & 0.893                    & 81,464                & 23.561                   & -22.667***                     \\
Num low downstream           & 1,247,784             & 1.362                    & 81,464                & 14.91                    & -13.549***                     \\
Num high entrep              & 1,247,784             & 1.405                    & 81,464                & 30.91                    & -29.505***                     \\
Num low entrep               & 1,247,784             & 0.85                     & 81,464                & 7.561                    & -6.711***                      \\
Pct serial entrep            & 478,021               & 27.627                   & 54,549                & 37.152                   & -9.525***                      \\
Pct serial entrep small      & 478,021               & 14.487                   & 54,549                & 29.536                   & -15.049***                     \\
Pct serial entrep large      & 478,021               & 21.116                   & 54,549                & 34.752                   & -13.635***                     \\
Tot shareholders             & 458,113               & 1.489                    & 53,683                & 1.736                    & -0.247***                      \\
Tot shareholders small       & 265,233               & 1.354                    & 45,559                & 1.579                    & -0.225***                      \\
Tot shareholders large       & 355,716               & 1.586                    & 51,185                & 1.815                    & -0.230***                      \\
Pct indiv shareholders       & 458,113               & 94.044                   & 53,683                & 89.503                   & 4.542***                       \\
Pct indiv shareholders small & 265,233               & 96.744                   & 45,559                & 94.475                   & 2.269***                       \\
Pct indiv shareholders large & 355,716               & 92.584                   & 51,185                & 87.273                   & 5.311***                       \\
Exec team size               & 426,589               & 2.054                    & 53,267                & 2.076                    & -0.023***                      \\
Exec team size small         & 231,887               & 1.994                    & 44,714                & 2.018                    & -0.024***                      \\
Exec team size large         & 341,686               & 2.101                    & 50,830                & 2.104                    & -0.003           \\
\bottomrule
